Massive-scale Decoding for Text Generation using Lattices

Conditional neural text generation models generate high-quality outputs, but often concentrate around a mode when what we really want is a diverse set of options. We present a search algorithm to construct lattices encoding a massive number of generation options. First, we restructure decoding as a best-first search, which explores the space differently than beam search and improves efficiency by avoiding pruning paths. Second, we revisit the idea of hypothesis recombination: we can identify pairs of similar generation candidates during search and merge them as an approximation. On both summarization and machine translation, we show that our algorithm encodes thousands of diverse options that remain grammatical and high-quality into one lattice. This algorithm provides a foundation for building downstream generation applications on top of massive-scale diverse outputs.

==> algo_recomb_base.tex <==

\algnewcommand\algorithmicrt{\textbf{return}}



% \begin{algorithm}
% \caption{Basic path recombination algorithm adopted from \cite{zhang-etal-2018-exploring}}
% \label{algo-recomb}
% \begin{algorithmic}[1]
% \Require  Equivalence function  $Eq(\cdot,\cdot)$, hypothesis score function $score(\cdot)$, one hypothesis chain $h$ existing in search frontier, one candidate hypothesis chain $h^{\prime}$.
% \Ensure Candidate hypothesis chain $h^{\prime}$ is recombined or not 
% \Procedure{Recomb}{$h,h^{\prime}$}
% % \Comment{The g.c.d. of a and b}
% \If{$Eq(h, h^{\prime})$ \textbf{and} $score(h) > score(h^{\prime})$}
%     \State $h$\texttt{.info} += ($h$, $h^{\prime}$)
%     \State \algorithmicrt{}  False \Comment{The information of $h^{\prime}$ is saved in $h$, and $h^{\prime}$ will not be added to the search frontier. }
% \Else
%     \State  \algorithmicrt{}  True \Comment{$h^{\prime}$ is added to the search frontier.}
% \EndIf
% \EndProcedure

% \end{algorithmic}
% \end{algorithm}


\begin{algorithm}
\caption{Improved path recombination algorithm based on Algo~\ref{algo-recomb}}
\label{algo-imp}
\begin{algorithmic}[1]
\Require \textcolor{gray}{  Equivalence function $Eq(\cdot,\cdot)$, hypothesis score function $score(\cdot)$, one hypothesis chain $h$ existing in search frontier, one candidate hypothesis chain $h^{\prime}$;} the ending node of $h$ is $n_{-1}$, the ending node of $h^{\prime}$ is $n_{-1}^{\prime}$.
\Ensure \textcolor{gray}{Candidate hypothesis chain $h^{\prime}$ is recombined or not}; updated successors of $h$.
\Procedure{RecombImp}{$h,h^{\prime}$}
% \Comment{The g.c.d. of a and b}
\If{$Eq(h_1, h_2)$ \textbf{and} $score(h) > score(h^{\prime})$}
    % \For{$\forall v: n_{-1} \in v\texttt{.prev} $   }
    \State $ n_{-1}\texttt{.prev}$ += [$n_{-2}^{\prime}$]
    % \EndFor
     \State \textcolor{gray}{ \algorithmicrt{}  False }
\Else
    \State \textcolor{gray}{ \algorithmicrt{}  True }
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figure_recomb.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure*}

\begin{algorithm}
\caption{Improved path recombination algorithm with Zip based on Algo~\ref{algo-imp}}
\begin{algorithmic}[1]
\Require \textcolor{gray}{  Equivalence function $Eq(\cdot,\cdot)$, hypothesis score function $score(\cdot)$, one hypothesis chain $h$ existing in search frontier, one candidate hypothesis chain $h^{\prime}$;} the ending node of $h$ is $n_{-1}$, the ending node of $h^{\prime}$ is $n_{-1}^{\prime}$.
\Ensure \textcolor{gray}{Candidate hypothesis chain $h^{\prime}$ is recombined or not}; updated successors of $h$.
\Procedure{RecombImp}{$h,h^{\prime}$}
% \Comment{The g.c.d. of a and b}
\If{$Eq(h_1, h_2)$ \textbf{and} $score(h) > score(h^{\prime})$}
    \State $z  \gets n_{-1}$ \Comment{$z$ stands for zip.}
     \State $z^{\prime}  \gets  n_{-1}^{\prime}$
   \While{ $z.token = z\prime .token $ }
        \State $z.prev$ += $z\prime.prev $
        \State $z.next$ += $z\prime.next$
        \Comment{We do not fork the unexpanded children of $z\prime$}
        \State $z \gets z.prev$; $z\prime \gets z\prime.prev$
   \EndWhile
   
    % \For{$\forall v: v \in z^{\prime}\texttt{.prev} $   }
    % \State $ z\texttt{.prev}$ += [$n_{-1}^{\prime}$]
    % \EndFor
     \State \textcolor{gray}{ \algorithmicrt{}  False }
\Else
    \State \textcolor{gray}{ \algorithmicrt{}  True }
\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> backup.tex <==


\begin{table*}[t]
\centering
\footnotesize
% \setlength{\tabcolsep}{6pt}
\begin{tabular}{@{}r|rrrrrr|ccccccc@{}} \toprule
        {}                    & \multicolumn{6}{c|}{\textsc{Diversity}}      & \tabgram & \multicolumn{3}{c}{\textsc{Oracle}} & \multicolumn{3}{c}{\textsc{Sample}} \\
     &
   &
$\uparrow$  &
$\uparrow$ &
 $\uparrow$ &
$\downarrow$ &
 $\uparrow$ &
$\downarrow$ &
   $\uparrow$ &
   $\uparrow$ &
   $\uparrow$ &
$\geq$ &
 $\geq$ &
  $\geq$ \\ 
Model &
  \numend &
\numpath  &
\novone &
 \novtwo &
\selfbleu &
  \edit & 
\errate &
  \multicolumn{1}{c}{R1} &
  \multicolumn{1}{c}{R2} &
  \multicolumn{1}{c}{RL} &
  \multicolumn{1}{c}{R1} &
  \multicolumn{1}{c}{R2} &
  \multicolumn{1}{c}{RL} \\ \midrule
\greedy                 & 1  & 1      & 22  & 23  & - & -  & 0.5\%                  & 41.4    & 17.3    & 33.5   & 41.4    & 17.3    & 33.5   \\
\bs                     & 16 & 16     & 40  & 57  & 89  & 30 & 0.4\%                  & 47.8    & 25.7    & 40.2   & 41.3    & 17.7    & 33.5   \\
\dbs                         & 16 & 16     & 54  & 81  & 82  & 52 & 0.5\%                  & 45.8    & 25.6    & 39.0   & 38.0    & 15.3    & 29.9   \\
\topp{0.8}                    & 16 & 16     & 111 & 202 & 59  & 71 & 0.6\%                  & 47.6    & 28.3    & 41.5   & 36.8    & 14.2    & 29.5   \\
\topp{0.9}                    & 16 & 16     & 127 & 232 & 56  & 74 & 0.7\%                  & 48.2    & 28.0    & 41.1   & 36.2    & 13.2    & 28.4   \\
\temp{1.5}                        & 16 & 16     & 150 & 269 & 51  & 81 & 1.3\%                 & 45.6    & 25.3    & 38.7   &  34.0    &  11.8    &  26.4   \\
\bfs                 & 30 & 30     & 88  & 167 & 68  & 60 & 0.4\%                  & 50.8     &  30.1   & 44.0  & 39.0    & 15.6    & 30.8   \\ \midrule
% \bfs post0.3         & 13 & 12     & 66  & 108 & 75  & 53 & 0.3\%                  & 48.1    & 27.5    & 41.1   & 38.7    & 15.3    & 30.3   \\ \midrule
\multicolumn{8}{l}{\textit{w. Path Recombination}} \\
 \bs \zhang  & 16 & 2,115  &  59  &  100 &   76  &   48 &    0.6\%                  & 51.8    & 31.7    & 44.9   & 40.0    & 16.3    & 32.4   \\
\rcb \topp{0.8}            & 13 & 52     & 167 & 308 & 53  & 79 & 1.0\%                  & 49.0    & 28.8    & 41.8   & 35.0    & 13.0    & 27.8   \\
\rcb \topp{0.9}             & 15 &36     &  207 &  363 &  50  &  87 &  1.7\%                  &   44.6    &   25.9    &   38.7   &   32.1    &   11.0    &   25.1   \\ 
\bfs \base      & 31 & 7,758  & 111 & 239 & 65  & 64 & 0.8\%                  & 55.2    & 35.8    & 49.3   &  38.5    & 15.2    & 30.8   \\
 \bfs \zip     &  33 &
  95,744 &
  124 &
  274 &
  53 &
  77 &
  1.4\% &
     55.6 &
     36.8 &
     48.8 &
  36.8 &
  13.2 &
  28.7  \\ \midrule
% \multicolumn{8}{l}{\textit{w. Path Recombination, 25\% budget}} \\
\textleaf  \bfs \zip   &  7 &
  297 &
  58 &
  92 &
  80 &
  49 &
  0.8\% &
  49.6 &
  29.2 &
  42.8 &
  38.8 &
  15.2 &
  31.0 \\ \bottomrule
\end{tabular}
\caption{Main results for all methods decoding text summaries on XSum. Diversity metrics are rounded to integer due to space limit. We use $\uparrow$, $\downarrow$ and $\geq$ to denote the desired trend, the higher the better, the lower the better, or good if it passes some threshold. Detailed explanation of metrics are listed in Sec.~\ref{sec-eval-met}. All our model use adhoc. }
\label{tab:xsum-main}
\end{table*}

